"Refsdal" meets Popper: comparing predictions of the re-appearance of the multiply imaged supernova behind MACSJ1149.5+2223

Supernova "Refsdal," multiply imaged by cluster MACSJ1149.5+2223, represents a rare opportunity to make a true blind test of model predictions in extragalactic astronomy, on a time scale that is short compared to a human lifetime. In order to take advantage of this event, we produced seven gravitational lens models with five independent methods, based on Hubble Space Telescope (HST) Hubble Frontier Field images, along with extensive spectroscopic follow-up observations by HST, the Very Large and the Keck Telescopes. We compare the model predictions and show that they agree reasonably well with the measured time delays and magnification ratios between the known images, even though these quantities were not used as input. This agreement is encouraging, considering that the models only provide statistical uncertainties, and do not include additional sources of uncertainties such as structure along the line of sight, cosmology, and the mass sheet degeneracy. We then present the model predictions for the other appearances of SN "Refsdal." A future image will reach its peak in the first half of 2016, while another image appeared between 1994 and 2004. The past image would have been too faint to be detected in existing archival images. The future image should be approximately one third as bright as the brightest known image (i.e., H_AB~25.7 mag at peak and H_AB~26.7 mag six months before peak), and thus detectable in single-orbit HST images. We will find out soon whether our predictions are correct.

==> authors.tex <==
% --------------------------------------------------
% Institutions
%   define a command for each institution's mailing address
% --------------------------------------------------
\newcommand{\HubbleFellow}{Hubble Fellow}
\newcommand{\Packard}{Packard Fellow}
\newcommand{\CalTech}{California Institute of Technology, 1200 East California Boulevard, Pasadena, CA 91125}
\newcommand{\Cantabria}{IFCA, Instituto de F\'isica de Cantabria (UC-CSIC), Av. de Los Castros s/n, 39005 Santander, Spain}
\newcommand{\IFCA}{\Cantabria}
\newcommand{\JHU}{Department of Physics and Astronomy, The Johns Hopkins University, 3400 N. Charles St., Baltimore, MD 21218, USA}
\newcommand{\Michigan}{Department of Astronomy, University of Michigan, 1085 S. University Avenue, Ann Arbor, MI 48109, USA}
\newcommand{\UCDavis}{University of California Davis, 1 Shields Avenue, Davis, CA 95616}
\newcommand{\UCLA}{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095}
\newcommand{\USC}{Department of Physics and Astronomy, University of South Carolina, 712 Main St., Columbia, SC 29208, USA}
\newcommand{\RCEU}{Research Center for the Early Universe, University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\TokyoPhys}{Department of Physics, University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\IPMU}{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU, WPI), University of Tokyo, 5-1-5 Kashiwanoha, Kashiwa, Chiba 277-8583, Japan}
\newcommand{\TokyoAstro}{Department of Astronomy, Graduate School of Science, The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\DARK}{Dark Cosmology Centre, Niels Bohr Institute, University of Copenhagen, Juliane Maries Vej 30, DK-2100 Copenhagen, Denmark} 
\newcommand{\INFN}{INFN, Sezione di Bologna, Viale Berti Pichat 6/2, I-40127 Bologna, Italy}
\newcommand{\EHU}{Fisika Teorikoa, Zientzia eta Teknologia Fakultatea, Euskal Herriko Unibertsitatea UPV/EHU}
\newcommand{\Basque}{IKERBASQUE, Basque Foundation for Science, Alameda Urquijo, 36-5 48008 Bilbao, Spain}
\newcommand{\Berkeley}{Department of Astronomy, University of California, Berkeley, CA 94720-3411, USA}
\newcommand{\STScI}{Space Telescope Science Institute, 3700 San Martin Dr., Baltimore, MD 21218, USA}
\newcommand{\Ferrara}{Dipartimento di Fisica e Scienze della Terra, Universit\`{a} degli Studi di Ferrara, via Saragat 1, I-44122, Ferrara, Italy}
\newcommand{\INAF}{INAF, Osservatorio Astronomico di Bologna, via Ranzani 1, I-40127 Bologna, Italy}
\newcommand{\UCSB}{Department of Physics, University of California, Santa Barbara, CA 93106-9530, USA}
\newcommand{\SantaBarbara}{\UCSB}
\newcommand{\Kapteyn}{Kapteyn Astronomical Institute, University of Groningen, Postbus 800, 9700 AV Groningen, the Netherlands}
\newcommand{\WKU}{Department of Physics, Western Kentucky University, Bowling Green, KY 42101, USA}
\newcommand{\IAP}{Institut d’Astrophysique de Paris, UMR7095 CNRS-Universit\'{e} Pierre et Marie Curie, 98bis bd Arago, F-75014 Paris, France}
\newcommand{\ASIAA}{Institute of Astronomy and Astrophysics, Academia Sinica, P.O. Box 23-141, Taipei 10617, Taiwan}
\newcommand{\TokyoKashiwa}{Institute for Cosmic Ray Research, The University of Tokyo, Kashiwa, Chiba 277-8582, Japan}
\newcommand{\Munich}{University Observatory Munich, Scheinerstrasse 1, D-81679 Munich, Germany} 

%\newcommand{\Chicago}{Department of Physics, The University of Chicago, Chicago, IL 60637, USA}
%\newcommand{\LBNL}{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
%\newcommand{\Riverside}{Department of Physics and Astronomy, University of California, Riverside, CA 92521, USA}
%\newcommand{\Andalucia}{Instituto de Astrof\'isica de Andaluc\'ia (CSIC), E-18080 Granada, Spain}
%\newcommand{\SaoPaulo}{Instituto de Astronomia, Geof\'isica e Ci\^encias Atmosf\'ericas, Universidade de S\~ao Paulo, Cidade Universit\'aria, 05508-090, S\~ao Paulo, Brazil}
%\newcommand{\AMNH}{Department of Astrophysics, American Museum of Natural History, Central Park West and 79th Street, New York, NY 10024, USA}
%\newcommand{\NYU}{Center for Cosmology and Particle Physics, New York University, New York, NY 10003, USA}
%\newcommand{\Copenhagen}{\DARK}
%\newcommand{\Arizona}{Department of Astronomy, University of Arizona, Tucson, AZ 85721, USA}
%\newcommand{\SantaCruz}{Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 92064, USA}
%\newcommand{\NotreDame}{Department of Physics, University of Notre Dame, Notre Dame, IN 46556, USA}
%\newcommand{\TelAviv}{Department of Astrophysics, Tel Aviv University, 69978 Tel Aviv, Israel}
\newcommand{\Rutgers}{Department of Physics and Astronomy, Rutgers, The State University of New Jersey, Piscataway, NJ 08854, USA}
%\newcommand{\CfA}{Harvard/Smithsonian Center for Astrophysics, Cambridge, MA 02138, USA}
%\newcommand{\Minnesota}{School of Physics and Astronomy, University of Minnesota, 116 Church Street SE, Minneapolis, MN 55455, USA}
%\newcommand{\NOAO}{National Optical Astronomical Observatory, Tucson, AZ 85719, USA}
%\newcommand{\LCOGT}{Las Cumbres Observatory Global Telescope Network, 6740 Cortona Dr., Suite 102, Goleta, California 93117, USA}
%\newcommand{\Colby}{Colby College, 4000 Mayflower Hill Dr, Waterville, ME 04901, USA}
%\newcommand{\Kentucky}{University of Kentucky, Lexington, KY 40506}
%\newcommand{\Durham}{Institute for Computational Cosmology, Durham University, South Road, Durham DH1 3LE, UK}
%\newcommand{\KwaZulu}{Astrophysics and Cosmology Research Unit, School of Mathematical Sciences, University of KwaZulu-Natal, Durban 4041, South Africa}
%\newcommand{\HongKong}{Department of Physics, The University of Hong Kong, Pokfulam Road, Hong Kong}
%\newcommand{\Oxford}{Department of Physics, University of Oxford, Keble Road, Oxford OX1 3RH, UK}
%\newcommand{\CRAL}{CRAL, Observatoire de Lyon, Universit\'e Lyon 1, 9 Avenue Ch. Andr\'e, F-69561 Saint Genis Laval Cedex, France}
%\newcommand{\Hebrew}{The Hebrew University, The Edmond J. Safra Campus - Givat Ram, Jerusalem 9190401, Israel}
\newcommand{\IllinoisAstro}{ Astronomy Department, University of Illinois at Urbana-Champaign, 1002 W.\ Green Street, Urbana, IL 61801, USA }
\newcommand{\IllinoisPhysics}{ Department of Physics, University of Illinois at Urbana-Champaign, 1110 W.\ Green Street, Urbana, IL 61801, USA }
%\newcommand{\JPL}{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA 91109, USA}



%\affil{$^{4}$ Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study (UTIAS), the University of Tokyo, Kashiwa, 277-8582, Japan}
%\affil{$^6$ Institute of Theoretical Astrophysics, University of Oslo, P.O. Box 1029, N-0315 Oslo, Norway}
%\affil{$^7$ The Observatories of the Carnegie Institution for Science, 813 Santa Barbara St., Pasadena, CA 91101, USA}
%\affil{$^{10}$ Astrophysics Science Division, Goddard Space Flight Center, Code 665, Greenbelt, MD 20771}
%\affil{$^{12}$ INAF-Astronomical Observatory of Padova, Italy}
%\affil{$^{13}$ School of Physics, University of Melbourne, VIC 3010, Australia%}
%\affil{$^{15}$ Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, 452 Lomita Mall, Stanford, CA  94305-4085, USA}



% --------------------------------------------------
% Author list 
%   use the \affilref and \affilreftxt commands 
%   to get an author list and footnoted institutional
%   addresses that count themselves without duplicating
% --------------------------------------------------
\newcounter{affilct}
\setcounter{affilct}{0}

% --------------------------------------------------
% \affilref{refcode}
%   Use this command inside each \altaffilmark{} instance.
%   It checks if the affiliation has already been used, and generates
%   a new affiliation reference number only if needed.
%   The user-defined refcode value will then be used by \affilreftxt
%   to set the same index number in the author list at the top and 
%   the footnoted list of institutional addresses. 
\makeatletter
\newcommand{\affilref}[1]{%
  \@ifundefined{c@#1}%
    {\newcounter{#1}%
     \setcounter{#1}{\theaffilct}%
     \refstepcounter{affilct}%
     \label{#1}%
     }{}%
  \ref{#1}%
 }
\makeatother


% --------------------------------------------------
% \affilreftxt{refcode}{address} : 
%   Use this command after each author definition 
%   to generate the footnote text containing one institutional
%   address for that author. 
%   It checks if the address has already been used, and generates
%   a new affiliation footnote with text only if needed.
\makeatletter
\newcommand*\affilreftxt[2]{%
  \@ifundefined{c@#1txt}
    {\newcounter{#1txt}%
     \setcounter{#1txt}{1}
     \altaffiltext{\ref{#1}}{#2}
     }{
     }
  }
\makeatother
% --------------------------------------------------


\author{T.~Treu\altaffilmark{\affilref{UCLA},\affilref{Packard}}}
\affilreftxt{UCLA}{\UCLA}
\affilreftxt{Packard}{\Packard}
\email{tt@astro.ucla.edu}

\author{G.~Brammer\altaffilmark{\affilref{STScI}}}
\affilreftxt{STScI}{\STScI}

\author{J.~M.~Diego\altaffilmark{\affilref{Cantabria}}}
\affilreftxt{Cantabria}{\Cantabria}

\author{C.~Grillo\altaffilmark{\affilref{DARK}}}
\affilreftxt{DARK}{\DARK}

\author{P.~L.~Kelly\altaffilmark{\affilref{Berkeley}}}
\affilreftxt{Berkeley}{\Berkeley}

\author{M.~Oguri\altaffilmark{\affilref{IPMU},\affilref{TokyoPhys},\affilref{RCEU}}}
\affilreftxt{IPMU}{\IPMU}
\affilreftxt{TokyoPhys}{\TokyoPhys}
\affilreftxt{RCEU}{\RCEU}

\author{S.~A.~Rodney\altaffilmark{\affilref{USC},\affilref{JHU},\affilref{HubbleFellow}}}
\affilreftxt{USC}{\USC}
\affilreftxt{JHU}{\JHU}
\affilreftxt{HubbleFellow}{\HubbleFellow}

\author{P.~Rosati\altaffilmark{\affilref{Ferrara}}}
\affilreftxt{Ferrara}{\Ferrara}

\author{K.~Sharon\altaffilmark{\affilref{Michigan}}}
\affilreftxt{Michigan}{\Michigan}

\author{A.~Zitrin\altaffilmark{\affilref{CalTech},\affilref{HubbleFellow}}}
\affilreftxt{CalTech}{\CalTech}

\author{I.~Balestra\altaffilmark{\affilref{Munich}}}
\affilreftxt{Munich}{\Munich}

\author{M. Brada\v{c}\altaffilmark{\affilref{UCDavis}}}
\affilreftxt{UCDavis}{\UCDavis}

\author{T.~Broadhurst\altaffilmark{\affilref{EHU},\affilref{Basque}}}
\affilreftxt{EHU}{\EHU}
\affilreftxt{Basque}{\Basque}

\author{G.~B.~Caminha\altaffilmark{\affilref{Ferrara}}}
\affilreftxt{Ferrara}{\Ferrara}

\author{M.~Ishigaki\altaffilmark{\affilref{TokyoKashiwa},\affilref{TokyoPhys}}}
\affilreftxt{TokyoKashiwa}{\TokyoKashiwa}
\affilreftxt{TokyoPhys}{\TokyoPhys}

%\author{R.~Gavazzi\altaffilmark{\affilref{IAP}}}
%\affilreftxt{IAP}{\IAP}

\author{T.~L.~Johnson\altaffilmark{\affilref{Michigan}}}
\affilreftxt{Michigan}{\Michigan}

\author{A.~Halkola}

\author{A.~Hoag\altaffilmark{\affilref{UCDavis}}}
\affilreftxt{UCDavis}{\UCDavis}

\author{W.~Karman\altaffilmark{\affilref{Kapteyn}}}
\affilreftxt{Kapteyn}{\Kapteyn}

\author{R.~Kawamata\altaffilmark{\affilref{TokyoAstro}}}
\affilreftxt{TokyoAstro}{\TokyoAstro}

\author{A.~Mercurio\altaffilmark{\affilref{INAF}}}
\affilreftxt{INAF}{\INAF}

%\author{X.~Wang\altaffilmark{\affilref{UCSB}}}
%\affilreftxt{UCSB}{\UCSB}

\author{K.~B.~Schmidt\altaffilmark{\affilref{UCSB}}}
\affilreftxt{UCSB}{\UCSB}

\author{L.-G.~Strolger\altaffilmark{\affilref{STScI},\affilref{WKU}}}
\affilreftxt{STScI}{\STScI}
\affilreftxt{WKU}{\WKU}

\author{S.~H.~Suyu\altaffilmark{\affilref{ASIAA}}}
\affilreftxt{ASIAA}{\ASIAA}

\author{A.~V.~Filippenko\altaffilmark{\affilref{Berkeley}}}
\affilreftxt{Berkeley}{\Berkeley}

\author{R.~J.~Foley\altaffilmark{\affilref{IllinoisAstro},\affilref{IllinoisPhysics}}}
\affilreftxt{IllinoisAstro}{\IllinoisAstro}
\affilreftxt{IllinoisPhysics}{\IllinoisPhysics}

\author{S.~W.~Jha\altaffilmark{\affilref{Rutgers}}}
\affilreftxt{Rutgers}{\Rutgers}

\author{B.~Patel\altaffilmark{\affilref{Rutgers}}}
\affilreftxt{Rutgers}{\Rutgers}








